Four Cometary Belts Associated with the Orbits of Giant Planets: A New View of the Outer Solar System's Structure Emerges from Numerical Simulations

Using numerical simulations, we examine the structure of a cometary population near a massive planet, such as a giant planet of the Solar system, starting with one-planet approximation (the Sun plus one planet). By studying the distributions of comets in semimajor axis, eccentricity, pericenter, and apocenter distances, we have revealed several interesting features in these distributions. The most remarkable ones include (i) spatial accumulation of comets near the planetary orbit (which we call the `cometary belt') and (ii) avoidance of resonant orbits by comets. Then we abandon one-planet approximation and examine as to how a cometary belt is modified when the influence of all four giant planets is taken into consideration. To this end, we simulate a stationary distribution of comets, which results from the gravitational scattering of the Kuiper belt objects on the four giant planets and accounts for the effects of mean motion resonances. Accounting for the influence of four giant planets makes the cometary belts overlapping, but nevertheless keeping almost all their basic features found in one-planet approximation. In particular, the belts maintain the gaps in the (a,e)- and (a,i)-space similar to the Kirkwood gaps in the main asteroid belt. We conclude that the large-scale structure of the Solar system is featured by the four cometary belts expected to contain 20-30 millions of scattered comets, and only a tiny fraction of them is currently visible as Jupiter-, Saturn-, etc. family comets.

==> ozerntab.tex <==

%++++++++++++++++++++++Table 1
%\input macro
\magnification=1200
%\raggedright
\pretolerance=10000  %no hyphenation
%%%%%%%%%% no number on first page.
\def\folio{\ifnum\pageno=1\nopagenumbers\else\number\pageno\fi}
%
%%%%%%%%%% fonts.
% Set up some definitions:  
%
%This is how to have an approximate sign under < or > :

\def\lax    {\ifmmode{_<\atop^{\sim}}\else{${_<\atop^{\sim}}$}\fi}
\def\gax    {\ifmmode{_>\atop^{\sim}}\else{${_>\atop^{\sim}}$}\fi}
\def\kms    {\ifmmode{{\rm ~km~s}^{-1}}\else{~km~s$^{-1}$}\fi}
\def\kmp    {~km~s$^{-1}$~pc$^{-1}$}
\def\lo     {~${\rm L}_{\odot}$}
\def\mo     {~${\rm M}_{\odot}$}
\def\moyr   {\hbox{~$M_{\odot}\,{\rm yr}^{-1}$}}
\def\etal   {{\sl et~al.~}}
\def\eg{{\it e.\thinspace g.~}}
\def\ie{{\it i.\thinspace e.~}}
\def\bk{\lower 6pt\hbox{${\buildrel k\over \sim}$}}
\def\bv{\lower 6pt\hbox{${\buildrel v\over \sim}$}}

\def\muas   {~$\mu${\rm as}}
\def\masyr  {~mas~yr$^{-1}$}
\def\htwoo  {~${\rm H_2O}$}
\def\vbot   {$V_\bot$}

%
%    (2) Define single-space command
%
\def\singlespace {\smallskipamount=3pt plus1pt minus1pt
		  \medskipamount=6pt plus2pt minus2pt
		  \bigskipamount=12pt plus4pt minus4pt
		  \normalbaselineskip=12pt plus4pt minus4pt
		  \normallineskip=1pt
		  \normallineskiplimit=0pt
		  \jot=3pt
		  {\def\smallskip {\vskip\smallskipamount}}
		  {\def\medskip   {\vskip\medskipamount}}
		  {\def\bigskip   {\vskip\bigskipamount}}
		  {\setbox\strutbox=\hbox{\vrule 
		    height8.5pt depth3.5pt width 0pt}}
		  \parskip 0pt
		  \normalbaselines}
%
%    (3) Double-spaced manuscript definition
%
\def\doublespace {\smallskipamount=6pt plus2pt minus2pt
		  \medskipamount=12pt plus4pt minus4pt
		  \bigskipamount=24pt plus8pt minus8pt
		  \normalbaselineskip=24pt plus8pt minus8pt
		  \normallineskip=2pt
		  \normallineskiplimit=0pt
		  \jot=6pt
		  {\def\smallskip {\vskip\smallskipamount}}
		  {\def\medskip   {\vskip\medskipamount}}
		  {\def\bigskip   {\vskip\bigskipamount}}
		  {\setbox\strutbox=\hbox{\vrule 
		    height17.0pt depth7.0pt width 0pt}}
		  \parskip 12.0pt
		  \normalbaselines}
%
\special{landscape}
\hsize 9 truein
\vsize 7 truein
\hoffset 0 truein
\voffset 0 truein
%
% Paragraph indenting, double spacing default
%
%\doublespace
\parindent 24.0pt
%
%7 August 1991 version
%
%
\def\blankline  {\vskip10truept}
\def\sal {\vskip 12 truept}
%\singlespace


\centerline{TABLE 1}
\medskip
\hrule
\medskip
\centerline{Details of Computational Runs}
\medskip
\hrule
\smallskip
\hrule
\medskip
\centerline{\vbox{
\halign{ \hfil # \hfil  & \hfil # \hfil  & \hfil # \hfil
& \hfil # \hfil  & \hfil # \hfil & \hfil # \hfil 
\cr
  & Neptune  & Uranus & Saturn  & Jupiter &
Four-planet approximation \cr
\noalign{\vskip 10pt}
 Number of runs  & 8 & 3 &  26 & 40 &36  \cr
\noalign{\vskip 10pt}
 Initial conditions$(^1)$: &  &  &   &  & \cr
%\noalign{\vskip 3pt}
$~~~~~a_0$ & 33 AU    & 21 AU & 10.5 AU & 5.7 AU 
& $39.27\leq a_0\leq 40.12$ AU  ~~~47.37 AU\cr
$~~~~~e_0$ & 0.11-0.14     & 0.11-0.14  & 0.11-0.14   & 0.11-0.14 
&  $0.24\leq e_0\leq 0.34$  ~~~~~0.38 \cr
$~~~~~i_0$ &  $5^\circ$   &  $5^\circ$   & 
 $5^\circ$   & $5^\circ$  
&  $1.4^\circ\leq i_0\leq 12.1^\circ$  ~~~~~$12.4^\circ$\cr
\noalign{\vskip 10pt}
%Number of planet's       & from $0.500\times 10^6$  & from 
% $0.76\times 10^6$ & from $1.69\times 10^4$  & from $1.50\times 10^3$  \cr
%\noalign{\vskip 3pt}
%revolutions during one run$(^1)$& to $0.985\times 10^6$    & to 
%$3.0\times 10^6$ & to $3.92\times 10^5$ & to $0.59\times 10^5$ \cr  
%\noalign{\vskip 10pt}
 Number of computed positions    & $1.05\times 10^6$    & $0.91\times 10^6$ 
  & $0.37\times 10^6$  & $0.77\times 10^5$ & $2.57\times 10^7$ \cr
\noalign{\vskip 10pt}
Time step (in planet's revolutions)  &  &  &  &  & \cr
%\noalign{\vskip 3pt}
 between making the record & 9.995  &  9.995 &  9.995 &  9.995 & 0.955  \cr
%\noalign{\vskip 3pt}
of the computed positions$(^2)$ & & & & & \cr
\noalign{\vskip 8pt}
}}}
\hrule
\bigskip

$(^1)$ taken so that the test bodies are not captured into 
resonances from the very beginning of the run. 
In the four-planet approximation, the initial conditions are taken, in 
accordance with observational data, near the resonances 3:2 and 2:1 with 
Neptune. The final distribution is
not sensitive to initial conditions, because the particle's motion becomes
chaotic very soon. 

$(^2)$ taken to be different from 10 or 1 in order to avoid the stroboscopic 
effect.


     
\end


